Trustless Audits without Revealing Data or Models

There is an increasing conflict between business incentives to hide models and data as trade secrets, and the societal need for algorithmic transparency. For example, a rightsholder wishing to know whether their copyrighted works have been used during training must convince the model provider to allow a third party to audit the model and data. Finding a mutually agreeable third party is difficult, and the associated costs often make this approach impractical. In this work, we show that it is possible to simultaneously allow model providers to keep their model weights (but not architecture) and data secret while allowing other parties to trustlessly audit model and data properties. We do this by designing a protocol called ZkAudit in which model providers publish cryptographic commitments of datasets and model weights, alongside a zero-knowledge proof (ZKP) certifying that published commitments are derived from training the model. Model providers can then respond to audit requests by privately computing any function F of the dataset (or model) and releasing the output of F alongside another ZKP certifying the correct execution of F. To enable ZkAudit, we develop new methods of computing ZKPs for SGD on modern neural nets for simple recommender systems and image classification models capable of high accuracies on ImageNet. Empirically, we show it is possible to provide trustless audits of DNNs, including copyright, censorship, and counterfactual audits with little to no loss in accuracy.

==> tex/apx_protocols.tex <==
\section{Applications of Verified ML Model Inference}
\label{sec:apx-protocols}

In this section, we describe our protocols for verifying ML models for different
applications. We describe our security model and our protocols for verifying ML
model predictions for audits, verifying ML model accuracy, and verifying ML
model predictions for serving.


\subsection{Protocol Properties and Security Model}

\minihead{Protocol properties}
In this section, we describe and study the properties of protocols leveraging
verified ML inference. Each protocol has a different set of requirements, which
we denote $A$. The requirements $A$ may be probabilistic (e.g., the model has
accuracy 80\% with 95\% probability). We are interested in studying the
\emph{validity} of our protocols, which states that if the protocol completes,
$A$ holds.

For the accuracy verification and inference protocols, the parties can choose to
participate or not. As such, we are also interested in the \emph{rational
participation} of our protocols, which states that economically rational actors
will participate in our protocols.


\minihead{Security model}
In this work, we use the standard ZK-SNARK security model for the ZK-SNARKs
\cite{bunz2020transparent}. Informally, the standard security model states the
prover and verifier only interact via the ZK-SNARKs and that the adversary is
computationally bounded. This excludes the possibility of side channels. This is
in contrast to prior work in MPCs, which assume a semi-honest adversary (i.e.,
adversaries that honestly follow the protocol). Namely, adversaries may be
malicious in our security model.

We further assume the standard security model of public, permissionless,
Turing-complete smart contract execution engines (which are typically
blockchains) \cite{mohanta2018overview}. Informally, two parties can securely
send messages and execute smart contracts publicly. 


\minihead{Assumptions}
We require standard assumptions for ZK-SNARKs and smart contract execution
engines for our protocols to be secure.

For validity, we require that it is hard to compute the order of random group
elements \cite{bunz2020transparent}, which is implied by the RSA assumption
\cite{rivest1978method}. We further require the difficulty of finding hash
collisions, which is standard in cryptography \cite{rogaway2004cryptographic}.
Namely, for validity, we only assume standard cryptographic assumptions.

For rational participation, we assume that all parties are economically rational
and that there is an escrow service. We note that this excludes ``griefing''
attacks, where a malicious party purposefully loses money to hurt another party.
We defer the analysis of non-economically rational actors to future work. The
escrow service can be constructed programmatically, such as via smart contracts.
Importantly, the escrow service can also be run permissionlessly and trustlessly.




\subsection{Verifying ML model predictions for audits}
In this setting, a requester is interested in retrieving records that match the
output of an ML model from a responder. The responder is is typically the
subject of a legal subpoena. For example, the requester may be a journalist
requesting documents under the Freedom of Information Act or the plaintiff
requesting documents for legal discovery. For this setting, we assume that the
requester has a model that has been validated by some external party, e.g., a
judge. The responder must divulge documents or images that match the ML model's
prediction for the positive class but wishes to keep the remainder of the
documents private.

The protocol proceeds as follows:
\begin{enumerate}
  \item The responder commits to the dataset by producing hashes of the documents.
  \label{audit:hash}
  \item The requester sends the model to the responder.
  \item The responder produces ZK-SNARKs of the model on the documents, with the
  inputs hashed. The responder sends the requester the documents that match the
  positive class of the model.
\end{enumerate}

The audit protocol guarantees the following: the responder will return the
documents from Stage \ref{audit:hash} that match the model's positive class.
The validity follows from the difficulty of finding hash collisions and the
security of ZK-SNARKs.

The responder may hash invalid documents (e.g., random or unrelated images),
which the protocol makes no guarantees over. This can be mitigated in several
ways, depending on the scenario.

For documents from a trusted source, the hashes can be verified from a signature
from the trusted source. As an example, hashes for government-produced documents
(in the FOIA setting) may be produced at the time of document creation.

For documents from an untrusted source (e.g., the legal discovery setting), we
require a commitment for the entire corpus. Given the commitment, the judge can
allow the requester to randomly sample a small number ($N$) of the documents to
verify the hashes. In this case, the requester can verify that the responder
tampered with at most $p = \exp\left( \frac{1 - \delta}{N} \right)$ for some
confidence level $\delta$.



\subsection{Verifying ML model accuracy}
In this setting, a model consumer (MC) is interested in verifying a model
provider's (MP) model's accuracy, and MP desires to keep the weights hidden.
As an example use case, MC may be interested in verifying the model accuracy to
purchase the model or to use MP as an ML-as-a-service provider (i.e., to
purchase predictions in the future). Since the weights are proprietary, MP
desires to keep the weights hidden.

For this setting, we are interested in analyzing both the validity and rational
participation. As such, we analyze the pseudononymous marketplace setting, where
there are many potential MCs and MPs. We assume the existence of an escrow
service. This escrow service need only be able to follow programmatic rules and
as a result can be done trustlessly via smart contracts
\cite{kurtulmus2018trustless}. Other forms of escrow services are also viable.

Denote the cost of obtaining a test input and label to be $E$, the cost of
ZK-SNARKing a single input to be $Z$, and $P$ to be the cost of performing
inference on a single data point. We enforce that $E > Z > P$. Furthermore, let
$N = N_1 + N_2$ be the number of examples used in the verification protocol.
These parameters are marketplace-wide and are related to the security of the
protocol.

The marketplace requires MP to stake $1000 N_1 E$ per model to participate. The
stake is used to prevent Sybil attacks, in which a single party fakes the
identity of many MPs. Given the stake, the verification protocol is as follows
for some accuracy target $a$:
\begin{enumerate}
  \item MP commits to an architecture and set of weights (by providing the
  ZK-SNARK keys and weight hash respectively). MC commits to a test set $\{
  (x_1, y_1), ..., (x_N, y_N) \}$ by publishing the hash of the examples.

  \item MP and MC escrows $2 N E + \epsilon$, where $\epsilon$ goes to the
  escrow service.

  \item MP selects a random subset of size $N_1$ of the test set. If MC aborts
  at this point, MC loses the full amount in the escrow to MP. If MC continues,
  it sends the subset of examples to MP.

  \item MP chooses to proceed or abort. If MP aborts, MC loses $N_1 P$ of the
  escrow to MP and the remainder of the funds are returned to MC and MP.
  \label{verify:mp-fooled}

  \item MC sends the remainder of the $N_2$ examples to MP. If MP aborts from
  here on out, MP loses the full amount in the escrow ($2 N E$) to MC.

  \item MP sends SNARKs of the $N_2$ examples with outputs revealed. The weights
  and inputs are hashed.

  \item If accuracy target $a$ is met, MC pays $2 (N_1 P + N_2 Z)$. Otherwise,
  MP loses the full amount $2NE$ to MC.
\end{enumerate}

The verification protocol is valid because MP must produce the outputs of the ML
model as enforced by the ZK-SNARKs. MC can compute the accuracy given the
outputs. Thus, if the protocol completes, the accuracy target is met.

Rational participation further requires that the cost of the model or price of
post-verification purchased predictions is greater than $1000 N_1 E$. Rational
participation requires that honest MP/MC will participate and that dishonest
MP/MC will not participate.
% TODO
% Our analysis below assumes that MP and MC do not ``time out.'' We defer the
% full protocol, which includes a sub-protocol to mitigate one of the parties
% timing out, to the Appendix.

Consider the case of an honest MP. If MC is dishonest, it can economically gain
by having MP proceed beyond Stage \ref{verify:mp-fooled} and having MP fail the
accuracy target. Since MP chooses the subsets $N_1$ and $N_2$, they can be drawn
uniformly from the full test set. Thus, MP can choose to proceed only if $P(a
\textrm{ met} | N_1) > 1 - \alpha$ is such that expected value for MP is
positive, where $\alpha$ depends on the choice of $\epsilon$ (we provide
concrete instantiations for $\alpha$ and $\epsilon$ below). If MC is honest, MP
gains in expected value by completing the protocol, as its expected gain is
\[
  (1 - \alpha) (N_1 P + 2 N_2 Z - \epsilon) + \alpha N_1 P.
\]

Consider the case of an honest MC. Note that an economically rational MP is
incentivized to serve the model if it has a model of high quality. Thus, we
assume dishonest MPs do not have model that achieves the accuracy target. The
dishonest MP can economically gain by aborting at Stage \ref{verify:mp-fooled}
at least 1000 times (as $E > P$). MC can choose to participate with MP that only
has a failure rate of at most 1\%. In order to fool honest MCs, MP must collude
to verify invalid test sets, which costs $2 \epsilon$ per verification. MP must
have 99 fake verifications for one failed verification from an honest MC. Thus,
by setting $\epsilon = \frac{N_1 P}{99}$, dishonest MP will not participate. For
this choice of $\epsilon$, $\alpha > \frac{49 N_1 P}{49 N_1 P + 99 NE}$.

From our analysis, we see that honest MP and MC are incentivized to participate
and that dishonest MP and MC will not participate, showing rational
participation.


\input{tex/tables/eval-main}


\subsection{Verifying ML Model Predictions}

In this setting, we assume that MC has verified model accuracy and is interested
in purchasing predictions in the ML-as-a-service setting. We use the same
notation as above.

The serving verification procedure proceeds in rounds of size $K$ (i.e.,
prediction is served over $K$ inputs). MC is allow to contest at any point
during the round, but not after the round has concluded. Furthermore, let $K
\geq K_1 > 0$. The verification procedure is as follows:
\begin{enumerate}
  \item MC escrows $2KZ$ and MP escrows $\beta KZ$, where $\beta \geq 2$ is
  decided between MP and MC.

  \item MC provides the hashes for the $K$ inputs to the escrow and sends the
  inputs to MP ($x_i$). MP verifies the hashes.

  \item MP provides the predictions ($y_i$) to the inputs (without ZK-SNARKs) to
  MC. MC provides the hash of $\textrm{Concat}(x_i, y_i)$ to the escrow.

  \item If MC believes MP is dishonest, MC can contest on any subset $K_1$ of
  the predictions.

  \item When contested, MP will provide the ZK-SNARKs for the $K_1$ predictions.
  If MP fails to provide the ZK-SNARKs, then it loses the full $\beta ZP$.

  \item If the ZK-SNARKs match the hashes, then MC loses $2 K_1 Z$ from the
  escrow and the remainder of the funds are returned. Otherwise, MP loses the
  full $\beta ZP$ to MC.
\end{enumerate}

For validity, if MP is honest, MC cannot contest successfully and the input and
weight hashes are provided. Similarly, if MC is honest and contests an invalid
prediction, MP will be unable to produce the ZK-SNARK.

% TODO: timeouts
For rational participation, first consider an honest MP. The honest MP is
indifferent to the escrow as it receives the funds back at the end of the round.
Furthermore, all contests by MC will be unsuccessful and MP gains $K_1 Z$ per
unsuccessful contest.

For honest MC to participate, they must either have a method of detecting
invalid predictions with probability $p$ or they can randomly contest a $p$
fraction of the predictions. Note that for random contests, $p$ depends on the
negative utility of MC receiving an invalid prediction. As long as $\beta KZ$ is
large relative to $\frac{K Z}{p}$, then MC will participate.


==> tex/impact.tex <==
\section{Impact Statement}

This paper presents work whose goal is to advance the field of Machine Learning.
There are many potential societal consequences of our work, none which we feel
must be specifically highlighted here.


==> tex/opts.tex <==
\section{Constructing ZK-SNARKs for ImageNet-Scale Models}
\label{sec:opts}

We now describe our main contribution, the implementation of a ZK-SNARK proof
for MobileNetv2 inference \cite{sandler2018mobilenetv2} in \texttt{halo2}. This
requires arithmetizing the building block operations in standard convolutional
neural networks (CNNs) in the Plonkish arithmetization. 


\subsection{Arithmetization}

Standard CNNs are composed of six distinct operations: convolutions, batch
normalization, ReLUs, residual connections, fully connected layers, and softmax.
We fuse the batch normalization into the convolutions and return the logits to
avoid executing softmax. We now describe our ingredients for constraining the
remaining four operations.

\minihead{Quantization and fixed-point}
DNN inference is typically done in floating-point arithmetic, which
is extremely expensive to emulate in the prime field of arithmetic circuits.
To avoid this overhead, we focus on DNNs quantized in \texttt{int8} and
\texttt{uint8}.  For these DNNs, weights and activations are represented as
8-bit integers, though intermediate computations may involve up to 32-bit integers.

In these quantized DNN, each weight, activation, and output is stored as a tuple
$(w_{\textrm{quant}}, z, s)$, where $w_{\textrm{quant}}$ and $z$ is an $8$-bit
integer weight and zero point, and $s$ is a floating point scale factor.  $z$
and $s$ are often shared for all weights in a layer, which reduces the number of
bits necessary to represent the DNN. In this representation, the
weight $w_{\textrm{quant}}$ represents the real number weight:
\[
w = (w_{\textrm{quant}} - z) \cdot s.
\]

To efficiently arithmetize the network, we replace the floating point $s$ by a
fixed point approximation $\frac{a}{b}$ for $a, b \in \mathbb{N}$ and compute
$w$ via 
\[
w = ((w_{\textrm{quant}} - z) \cdot a) / b.
\]
The intermediate
arithmetic is done in standard 32-bit integer arithmetic. 
% Our choice of lower
% precision values of $a$ and $b$ results in a slight accuracy drop but dramatic
% improvements in prover and verifier performance.

As an example of fixed point arithmetic after this conversion, consider adding
$y = x_1 + x_2$ with zero points and scale factors $z_y, z_1, z_2$ and $s_y, s_1, s_2$,
respectively. The floating point computation
\[
  (y - z_y) \cdot s_y = (x_1 - z_1) \cdot s_1 + (x_2 - z_2) \cdot s_2
\]
is replaced by the fixed point computation 
\[
  y \approx (x_1 - z_2) \cdot \frac{a_1}{b_1} \frac{b_y}{a_y} + (x_2 - z_2)
  \cdot \frac{a_2}{b_2} \frac{b_y}{a_y} + z_y.
\]
The addition and multiplication can be done natively in the field, but the
division cannot. To address this, we factor the computation of each layer into
dot products and create a custom gate to verify division. We further fuse the
division and non-linearity gates for efficiency.



\minihead{Custom gates for linear layers}
MobileNets contain three linear layers (layers with only linear operations):
convolutions, residual connections, and fully connected layers. For these linear
layers, we perform the computation per activation. To avoid expensive floating
point scaling by the scale factor and the non-linearities, we combine these
operations into a single sub-circuit.

To reduce the number of custom gates, we only use two custom gates for all
convolutions, residual connections, and fully connected layers. The first
custom gate constrains the addition of a fixed number of inputs $x^j_i$ in row $i$
via $c_i = \sum_{j = 1}^N x^j_i$.

%
The second custom gate constrains a dot product \emph{of fixed size} with a zero
point. For constant zero point $z$, inputs $x^j_i$, weights $w^j_i$, and output
$c_i$ in row $i$, the gate implements the polynomial constraint
\[
c_i = \sum_{j=1}^N (x^j_i - z) \cdot w^j_i
\]
for a fixed $N$.  To implement dot products of length $k < N$, we constrain
$w_{k + 1}, \ldots, w_N = 0$.  For dot products of length $k > N$, we use copy
constraints and the addition gate.

While the addition gate can be represented with the dot product gate, we use
two gates for efficiency. Namely, the custom addition gate can perform
an N-element addition using half as many grid cells as the dot product gate.

\minihead{Lookup arguments for non-linearities}
Consider the result of an unscaled, flattened convolution:
$
c_i = \sum_j x^j_i \cdot w^j_i,
$
where $j$ indexes over the image height, width, and channels, and $i$ is the row. Performing
scale factor division and (clipped) ReLU to obtain the final activation
requires computing
\[
a_i = \text{ClipAndScale}(c_i, a; b)
:= \textrm{clip}\Big(\left\lfloor \frac{c_i \cdot a}{b} \right\rfloor, 0, 255\Big).
\]
To constrain this efficiently, we apply a lookup argument and use the same value
of $b$ across layers. To do so, we first perform the division by $b$ using a
custom gate. Since $b$ is fixed, we can use the same custom gate and lookup
argument. Let $d_i = \frac{c_i \cdot a}{b}$. We then precompute the possible
values of the input/output pairs of $(d_i, a_i)$ to form a lookup table
\[
T = \{(c, \text{ClipAndScale}(c)) \mid c \in \{ 0, \ldots, N \}\}.
\]
$N$ is chosen to
cover the domain, namely the possible values of $c$. We then use a lookup
argument to enforce the constraint $\textrm{Lookup}[(d_i, a_i) \in T]$.

We emphasize that naively using lookup arguments would result in a different
lookup argument per layer since the scale factors differ. Using different
lookup arguments would add high overhead, which our approach avoids. Sharing
lookups can result in small accuracy losses (e.g., as little as 0.1\%) but can
save over 2$\times$ the computational burden.


\minihead{Automated translation from TensorFlow Lite}
We created a translation layer to compile TensorFlow Lite models into circuits in the
\texttt{halo2} software package.  The translation layer automatically unrolls the
inference computation into an arithmetic circuit in the Plonkish arithmetization using
the custom gate and lookup arguments described above.

Our translation layer implements two optimizations. First, to minimize the
number of columns and the number of custom gates, our translation layer packs as
many operations as possible within a row. Second, we reduce the number of lookup
arguments by sharing lookup tables between layers when the scale factors are the
same. This is particularly useful for the residual layers, where the scaling
factor can be normalized to be shared across layers.


\subsection{Committing to weights or inputs}

ZK-SNARKs allow parts of the inputs to be made public, in addition to revealing
the outputs of the computation (Section~\ref{sec:snarks}). For ML models, the
input (e.g., image), weights, or both can be made public.  Then, to commit to
the hidden inputs, the hash can be computed within the ZK-SNARK and be made
public.  Concretely, we use the following primitives: 1) hidden input, public
weights, 2) public input, hidden weights, and 3) hidden input, hidden weights. 
% \begin{enumerate}[topsep=0.1em, leftmargin=1.3em]
%   \item \textbf{Hidden input, public weights}
%   % : the input is hidden and the
%   % weights are public. The input hash is computed and made public.
%   \item \textbf{Public input, hidden weights}
%   % : the input is public and the
%   % weights are hidden. The weight hash is computed and made public.
%   \item \textbf{Hidden input, hidden weights}
%   % : the inputs and weights are
%   %hidden. The hashes of both are computed and made public.
% \end{enumerate}
Commitments to all hidden parts are made public. We use an existing circuit for the SNARK-friendly Poseidon hash
\cite{grassi2019poseidon}.


==> tex/snarks.tex <==
\section{ZK-SNARKs}
\label{sec:snarks}

\minihead{Overview}
Consider the task of verifying a function evaluation $y = f(x; w)$ with
\emph{public inputs} $x$, \emph{private inputs} $w$, and output $y$. In the
setting of public input and hidden model, $x$ is an image, $w$ is the weights of
a DNN, and $y$ is the result of executing the DNN with weights $w$ on $x$.

A ZK-SNARK \cite{bitansky2017hunting} is a cryptographic protocol allowing a
Prover to generate a proof $\pi$ so that with knowledge of $\pi$, $y$, and $x$
alone, a Verifier can check that the Prover knows some $w$ so that $y = f(x;
w)$. ZK-SNARK protocols satisfy non-intuitive properties summarized
informally below:
%
\begin{enumerate}% [topsep=0.1em, leftmargin=1.3em, itemsep=0em]
  \item \emph{Succinctness}: The proof size is sub-linear (typically constant or
  logarithmic) in the size of the computation (i.e., the complexity of $f$).
  \item \emph{Non-interactivity}: Proof generation does not require interaction
  between the verifier and prover.
  \item \emph{Knowledge soundness}: A computationally bounded prover cannot
  generate proofs for incorrect executions.
  \item \emph{Completeness}: Proofs of correct execution verify.
  \item \emph{Zero-knowledge}: $\pi$ reveals no information about
  $w$ beyond what is contained in the output and $x$.
\end{enumerate}

Most ZK-SNARK protocols proceed in two steps. In the first step, called
\emph{arithmetization}, they produce a system of polynomial equations over a
large prime field (an arithmetic circuit) so that finding a solution is
equivalent to computing $f(x; w)$. Namely, for $(f, y, x, w)$, the circuit
constraints are met if and only if $y = f(x; w)$. In the second step, a
cryptographic \emph{proof system}, often called a \emph{backend},
generates a ZK-SNARK proof. 

This work uses the Halo2 ZK-SNARK protocol \cite{halo2} implemented in the
\texttt{halo2} software package.  In contrast to ZK-SNARK schemes custom
designed for neural networks in prior work \cite{liu2021zkcnn, lee2020vcnn},
Halo2 is designed for general-purpose computation, and \texttt{halo2} has a
broader developer ecosystem.  This means we inherit the security,
efficiency, and usability of the resulting developer tooling.  In the remainder
of this section, we describe the arithmetization and other properties of Halo2.

\minihead{Plonkish arithmetization}
Halo2 uses the Plonkish arithmetization \cite{halo2}, which allows polynomial
constraints and certain restricted forms of randomness. It is a special case of
a randomized AIR (Arithmetic Intermediate Representation) with preprocessing
\cite{bensasson2018scalable, gabizon2021from} which unifies recent proof systems
\cite{gabizon2019plonk, gabizon2020plookup, pearson2022plonkup}.

% a subset of randomized
% AIR with preprocessing \cite{bensasson2018scalable, gabizon2021from} unifying
% the recent proof systems PlonK, plookup, and PlonKup
% \cite{gabizon2019plonk, gabizon2020plookup, pearson2022plonkup}.

Variables in the arithmetic circuit are arranged in a rectangular grid with
cells valued in a $254$-bit prime field. The Plonkish arithmetization allows
three types of constraints:

% \footnote{Arbitrary computation can be expressed, but the size of the
% circuit depends on the nature of the computation.}

\emph{Custom gates} are polynomial expressions over cells in a single row that
must vanish on \emph{all} rows of the grid. As an example, consider a grid
with columns labeled $a, b, c$ with $a_i, b_i, c_i$ being the cells in row $i$.
The custom \emph{multiplication gate}
$a_i \cdot b_i - c_i = 0$
enforces that $c_i = a_i \cdot b_i$ for all rows $i$.

In nearly all circuits, it is beneficial to have custom gates only apply to
specific rows. To do this, we can add an extra column $q$ (per custom gate),
where each cell in $q$ takes the value 0 or 1; $q$ is called a selector. Then,
we can modify the custom gate to only apply for rows where $q_i \neq 0$:
$
q_i \cdot (a_i \cdot b_i - c_i) = 0.
$

\emph{Permutation arguments} allow us to constrain pairs of cells to have equal
values. They are used to copy values from one cell to another.  They are
implemented via randomized polynomial constraints for \emph{multiset} equality
checks.
  
\emph{Lookup arguments} allow us to constrain a $k$-tuple of cells $(d^1_i,
\ldots, d^k_i)$ in the same row $i$ with the following constraint. For a
disjoint set of $k$ other columns, the cells $(d^1_i, \ldots, d^k_i)$ must match
the values in some other row $i'$. Namely, we can constrain $(d^1_i, \ldots,
d^k_i) = (e^{1'}_{i'}, \ldots, e^{k'}_{i'})$. This constrains $(d^1_i, \ldots,
d^k_i)$ to lie in the \emph{lookup table} defined by those $k$ other columns. We
use lookup arguments in the arithmetization in two ways.  First, we implement
range checks on a cell $c$ by constraining it to take values in a fixed range
$\{0, \ldots, N - 1\}$. Second, we implement non-linearities by looking up a
pair of cells $(a, b)$ in a table defined by exhaustive evaluation of the
non-linearity. Lookup arguments are also implemented by randomized polynomial
constraints. 

\vspace{0.5em}

Prior work on SNARK-ing neural networks using proof systems intended for generic
computations started with the more limited R1CS arithmetization
\cite{gennaro2013quadratic} and the Groth16 proof system \cite{groth2016size},
in which DNN inference is less efficient to express. In Section \ref{sec:opts},
we describe how to use this more expressive Plonkish arithmetization to
efficiently express DNN inference.


\minihead{Performance for Halo2 circuits}
Halo2 is a polynomial interactive oracle proof (IOP)
\cite{bensasson2016interactive} made non-interactive via the Fiat-Shamir
heuristic. In a polynomial IOP, the ZK-SNARK is constructed from column
polynomials which interpolate the values in each column.  In Halo2, these
polynomials are fed into the \emph{inner product argument} introduced by
\citet{bowe2019recursive} to generate the final ZK-SNARK.

Several aspects of performance matter when evaluating a ZK-SNARK proof for a
computation. First, we wish to minimize proving time for the Prover and
verification time for the Verifier.  Second, on both sides, we wish to minimize
the proof size. All of  these measures increases with the number of rows,
columns, custom gates, permutation arguments, and lookup arguments.

%Although a precise cost model for these is complex in Halo2, all
%of these measures generally increase with the number of rows, columns, custom
%gates, permutation arguments, and lookup arguments.


==> tex/tables/eval-main.tex <==
\begin{table*}[t!]
% \small
\centering
\begin{tabular}{llllll}
%
Model & Accuracy (top-5) & Setup time & Proving time & Verification time & Proof
size (bytes) \\
\hline
MobileNet, 0.35, 96  & 59.1\% & 49.1 s  & 92.0 s  & 0.23 s & 5984 \\
MobileNet, 0.5, 224  & 75.7\% & 455.5 s & 831.9 s & 2.32 s & 7008 \\
MobileNet, 0.75, 192 & 79.2\% & 571.7 s & 850.7 s & 3.23 s & 5408
%
\end{tabular}
%
% \vspace{-0.75em}
\caption{Accuracy, setup time, proving time, and verification time of MobileNet
v2s. The first parameter is the ``expansion size'' parameter for the MobileNet
and the second parameter is image resolution. It is now possible to SNARK
ImageNet models, which no prior work can achieve.}
% \vspace{-0.5em}
%
\label{table:eval}
%
\end{table*}

